John Michael Hammersley (1920-2004)

In writing this biographical memoir of John Hammersley, we have tried to communicate something of the character of the person, and of the impact of his scientific achievements across lattice models (for example, percolation, self-avoiding walks, first-passage percolation, dimer models), stochastic processes (including subadditive ergodic theory), Monte Carlo methods, applied probability, statistics, and other areas to which he contributed. There is also an extended account of his earlier life, taken from autobiographical notes written around 1994, together with a list of his published work.

==> jmhlab.tex <==
\ifx\labelsloaded\relax\endinput\else\let\labelsloaded\relax\fi
\catcode`\@=11 % Letter
%
\newwrite\@auxout
\newif\if@fwdref \@fwdreffalse
 
%      **************************
%      *       COUNTERS         *
%      **************************
%
\newcount\Thm@nro \Thm@nro=0
\newcount\Sec@nro \Sec@nro=0
\newcount\SubSec@nro \SubSec@nro=0
\newcount\Item@nro \Item@nro=0
%
\def\theThm{\the\Thm@nro}
\def\theSec{\the\Sec@nro}
\def\theSubSec{\the\SubSec@nro}
\def\theItem{\the\Item@nro}
%
%
\def\stepbyone#1{\global\expandafter
  \advance\csname#1@nro\endcsname by1\relax}
\def\stepcounter#1#2{\global\expandafter
  \advance\csname#1@nro\endcsname by #2\relax}
\def\setcounter#1#2{\global\expandafter\csname#1@nro\endcsname =#2\relax}
\def\setcountern#1#2{\global\expandafter\csname#1@num\endcsname =#2\relax}

\def\Thm@#1{\xdef\@currentlabel{#1 \LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 A.\theThm
	 \else
    		\ifnum\SubSec@nro=0 \theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm}%
  \xdef\@heading{%
    \LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 A.\theThm
	 \else
    		\ifnum\SubSec@nro=0 \theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm%
   \ {\smc #1.\ }}\@heading} %GRG
\def\Thm#1{\stepbyone{Thm}\Thm@{#1}}

\def\Sec@#1{\setcounter{SubSec}0\setcounter{Thm}0%
   \xdef\@currentlabel{Section \ifnum\Sec@nro=0\else\theSec\fi}
   \xdef\@currentcontentsentry{#1}
  \xdef\@heading{%
    \ifnum\Sec@nro=0\else\theSec\fi}\@heading}
\def\Sec#1{\stepbyone{Sec}\Sec@{#1}}

\def\SubSec@{\setcounter{Thm}0%
\xdef\@currentlabel{Section\ifnum\SubSec@nro=0\else \theSec.\theSubSec\fi}%
\xdef\@heading{\ifnum\SubSec@nro=0\else \theSec.\theSubSec\fi}\@heading}

\def\SubSec{\stepbyone{SubSec}\SubSec@}

\def\Item@{\xdef\@currentlabel{\LeftTagForm
    \ifnum\Item@nro=0 \else\romannumeral\theItem\fi\RightTagForm}%
  \@currentlabel}
\def\Item{\stepbyone{Item}\Item@}

\def\appendix#1{\setcounter{Sec}0\vskip0.25in\centerline{\bf Appendix. #1}\bigskip\flushpar\is}
\def\section#1#2{\goodbreak\vskip0.25in\goodbreak\centerline{\bf\Sec{#2}. #2}
   \nobreak\medskip\nobreak\flushpar\is\label{#1}}
\def\subsection#1#2{\medskip\line{\hbox{{\it\SubSec. #2}}\hfill}
 \nobreak\smallskip\nobreak\flushpar\is\label{#1}}

\comment
%\def\proclaim#1#2#3{\setcounter{Item}0\smallskip\goodbreak
%   \thmskip\flushpar\Thm{#3}\label{#1}{\it #2}\nobreak\smallskip\nobreak\flushpar}
\def\cor#1#2{\proclaim{#1}{#2}{Corollary}}
\def\defn#1#2{\proclaim{#1}{#2}{Definition}}
\def\lemma#1#2{\proclaim{#1}{#2}{Lemma}}
\def\note#1#2{\proclaim{#1}{#2}{Note}}
\def\prop#1#2{\proclaim{#1}{#2}{Proposition}}
\def\thm#1#2{\proclaim{#1}{#2}{Theorem}}
\def\proof{\smallskip\flushpar{\smc Proof.}\quad}
\def\sketchproof{\smallskip\flushpar{\smc Sketch Proof.}\quad}
\def\temp#1{\smallskip\flushpar{\hbox{{\smc Temporary details:}} #1}{\hfil$\spadesuit$\linebreak}\flushpar}
\def\thmskip{\vskip10pt}
\endcomment

%\def\item#1#2{\flushpar{\hbox{\hbox to1cm{\rm\Item}\label{#1}\hfil} #2\hfil}}
\def\Proofitem#1#2{\flushpar{\hbox{\refer{#1}} #2}\flushpar}

\def\LeftTagForm{(}
\def\RightTagForm{)}
\def\Tag@{\xdef\@currentlabel{\LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 A.\theThm
	 \else
    		\ifnum\SubSec@nro=0 \theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm}%
  \@currentlabel}
\def\Tag{\stepbyone{Thm}\Tag@}
 
%\catcode`\@=\active
%
%   END EDITING
%================================================================
 
%    ********************************
%    *   CROSS REFERENCING MACROS   *
%    ********************************
%
%  The user writes  \label{foo}  to define the following cross-references:
%     \ref{foo}     : value of most recently incremented referencable counter.
%       (Chapter, section, theorem, tag, figure, table and roster's item
%        counters are referencable, footnote counters are not.)
%     \pageref{foo} : page number at which \label{foo} command appeared.
%  where  foo  can be any string of characters not containing '\', '{' or '}'.
%
 
\def\thepage{\number\pageno}
 
\def\refer#1{\@ifundefined{r@#1}{{ ??}\global\@fwdreftrue\@warning
   {Reference `#1' on page \thepage \space
    undefined}}{\edef\@tempa{\@nameuse{r@#1}}\expandafter
    \@car\@tempa \@nil\null}}
 
\def\referpage#1{\@ifundefined{r@#1}{{ ??}\global\@fwdreftrue\@warning
   {Reference `#1' on page \thepage \space
    undefined}}{\edef\@tempa{\@nameuse{r@#1}}\expandafter
    \@cdr\@tempa\@nil\null}}
 
\newif\if@filesw \@fileswtrue
 
\def\label#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
\def\contentsentry#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newcontentsentry{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
 
% \rosterlabel is AmSTeX-specific
\def\rosterlabel#1{\@bsphack\xdef\@currentlabel{%
   \therosteritem{\number\rostercount@}}%
   \if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
\def\newlabel#1#2{\@ifundefined{r@#1}{}{\@warning{Label `#1' multiply
   defined}}\global\@namedef{r@#1}{#2}}
 
\def\@currentlabel{} % For \label commands that come before any environment
 
%     ****************
%     *   INDEXing   *
%     ****************
% This is quite primitive
%
\newif\if@indexsw
\newwrite\@idxout
 
\def\makeindex{\@indexswtrue\immediate\openout\@idxout=\jobname.idx
   \immediate\write\@idxout{\string\relax}}
 
\def\index#1{\@bsphack\if@indexsw {\let\thepage\relax
   \xdef\@gtempa{\write\@idxout{\string
      \indexentry{#1}{\thepage}}}}\@gtempa
   \fi\@esphack}
 
\def\indexentry#1#2{\noindent {#1}{\unskip\nobreak\hfil\penalty50
   \hskip2em\hbox{}\nobreak\hfil#2%
   \parfillskip=0pt \finalhyphendemerits=0 \par}}
 
%      **************************
%      *       CITATIONS        *
%      **************************
%      These are AmS-TeX specific
%
%  CONVENTION
%  \b@FOO : The name or number of the reference created by \citeto{FOO}
%     E.g., if \citeto{FOO} -> [17] , then \b@FOO -> 17.
%
\def\make@ref#1{\@ifundefined{b@#1}{{??}\global\@fwdreftrue\@warning
   {Citation `#1' on page \thepage \space
    undefined}}{\@nameuse{b@#1}}}
%
% FROM AMSTEX.TEX
%\newif\ifin@
%\def\in@#1#2{\def\in@@##1#1##2##3\in@@{\ifx\in@##2\in@false\else\in@true\fi}%
% \in@@#2#1\in@\in@@}
%
\def\citeto#1{\relaxnext@
 \def\nextiii@##1,##2\end@{\immediate\write\@auxout{\string\citation{##1}}%
   {\make@ref{##1}},##2}%
 \in@,{#1}\ifin@\def\next{\nextiii@#1\end@}\else
   \def\next{\immediate\write\@auxout{\string\citation{#1}}%
     {\make@ref{#1}}}\fi
     \next}
\def\noOf#1{\global\advance\c@num by1
   \if@filesw \immediate\write\@auxout
   {\string\bibcite{#1}{\the\c@num}}\fi\no\make@ref{#1}}
\def\keyOf#1#2{\if@filesw
   {\def\protect##1{\string ##1\space}\immediate
   \write\@auxout{\string\bibcite{#1}{#2}}}\fi
   \key{{#2}}}
 
\def\TAG{\tag"\Tag"}
% AmSTeXin pitaa joissakin komennoissaan voida nahda \tag suoraan
% joilloin komentoa \TAG ei voi kayttaa, vaan tulee kirjoittaa \tag"\Tag"
% Tassa pitaa kayttaa AmSTeXin \tagin literaalista optiota \tag"...",
% silla numerossa \Tag ovat sulut (...) mukana.
% Jos sulkujen muotoa halutaan muuttaa, ovat sulut maariteltyna nimilla
% \LeftTagForm (vasen kaarisulku) ja \RightTagForm (oikea kaarisulku).
% Siis: \redefine\LeftTagForm{...} (tarvittaessa \predefine ...).
% ==========================================================================
\let\@@end=\end
\let\@@supereject=\supereject
\def\supereject{\@@supereject}
\def\end{\if@fwdref
  \typeout{Undefined forward references/citations. Rerun.}\fi
  \@@end}
%
% PLAINin \bye
%\def\bye{\par\vfill\supereject\end}
%
% AMSTEXin \enddocument
%\outer\def\enddocument{\nobreak\sfcode`\.=3000 \vskip12\p@ minus6\p@
% \thekeywords@\thesubjclass@\nobreak\vskip12\p@ minus6\p@\addressnum@\z@
% \loop\ifnum\addressnum@<\addresscount@\advance\addressnum@\@ne
% \csname address\number\addressnum@\endcsname\repeat
% \vfill\supereject\end}
 
%      **************************
%      *     USEFUL HACKS       *
%      **************************
%
%  \@namedef{NAME}   : Expands to \def\NAME , except name can contain any
%         characters.
%  \@nameuse{NAME}   : Expands to \NAME .
%  \@ifnextchar X{YES}{NO}
%       : Expands to YES if next character is an 'X',
%         and to NO otherwise. (Uses temps a-c.)
%         NOTE: GOBBLES ANY SPACE FOLLOWING IT.
%  \@ifundefined{NAME}{YES}{NO}
%       : If \NAME is undefined then it executes YES,
%         otherwise it executes NO.  More precisely,
%         true if \NAME either undefined or = \relax.
%  \@car T1 T2 ... Tn\@nil == T1  (unexpanded)
%  \@cdr T1 T2 ... Tn\@nil == T2 ... Tn     (unexpanded)
%  \typeout{message} : produces a warning message on the terminal
%  \@warning{message}: prints 'Warning: message.'
%
\newwrite\@unused
\def\typeout#1{{\let\protect\string\immediate\write\@unused{#1}}}
\def\@warning#1{\typeout{Warning: #1.}}
 
\def\@namedef#1{\expandafter\def\csname #1\endcsname}
\def\@nameuse#1{\csname #1\endcsname}
 
\def\@car#1#2\@nil{#1}
\def\@cdr#1#2\@nil{#2}
 
\long\def\@ifundefined#1#2#3{\expandafter\ifx\csname
  #1\endcsname\relax#2\else#3\fi}
 
\def\@ifnextchar#1#2#3{\let\@tempe #1\def\@tempa{#2}\def\@tempb{#3}\futurelet
    \@tempc\@ifnch}
\def\@ifnch{\ifx \@tempc \@sptoken \let\@tempd\@xifnch
      \else \ifx \@tempc \@tempe\let\@tempd\@tempa\else\let\@tempd\@tempb\fi
      \fi \@tempd}
 
\def\?{\let\@sptoken= } \?  % this makes \@sptoken a space token
 
\def\?{\@xifnch} \expandafter\def\? {\futurelet\@tempc\@ifnch}
 
% SPACE HACKS
% \@bsphack ... \@esphack
%     used by macros such as \index and \label
%     that want to be invisible -- i.e.,
%     not leave any extra space when used in the middle of text.  Such
%     a macro should begin with \@bsphack and end with \@esphack
%     The macro in question should not create any text, nor change the
%     mode.
%
\newdimen\@savsk
\newcount\@savsf
 
\def\@bsphack{\@savsk\lastskip
    \ifhmode\@savsf\spacefactor\fi}
 
\def\@esphack{\relax\ifhmode\spacefactor\@savsf
     {}\ifdim \@savsk >\z@ \ignorespaces\fi\fi}
 
%     **************************
%     *    FILE HANDLING       *
%     **************************
%
%    \Input{foo} : If file foo exists, then \input's it,
%                  otherwise types a warning message.
\def\Input#1{\openin1 #1 \ifeof1 \typeout{No file #1.}\closein1
    \else\closein1 \relax\input #1 \fi}
 
%      **************************
%      *     BIBLIOGRAPHY       *
%      **************************
%
\newcount\c@num \c@num=0
\def\reset{\setcountern{c}0}

\def\bibcite#1#2{\@ifundefined{r@#1}{}{\@warning{Referencelabel `#1' multiply
   defined}}\global\@namedef{b@#1}{#2}}
 
\def\@gobble#1{}
\let\citation\@gobble
 
%      **************************
%      *      INSERTIONS        *
%      **************************
%
% AMSTEX.TEXin \ins@ (\midspace...) MUUTETTU
%
% Jos \ins@:n \caption ulottuu kahdelle riville
% tulisi \captionissa mahd. esiintyva \Fig sovellettua
% kahdesti ja \Fig-numero kasvaisi kahdella
%
\def\CorrectCounter{}
%\newif\ifmid@
%\def\topspace{\mid@false\ins@}
%\def\midspace{\mid@true\ins@}
\def\ins@#1{\relaxnext@
 \smallcaptionwidth@\captionwidth@\gdef\thespace@{#1}%
 \def\next@{\ifx\next\space@\def\next. {\futurelet\next\nextii@}\else
  \def\next.{\futurelet\next\nextii@}\fi\next.}%
 \def\nextii@{\ifx\next\caption\def\next\caption{\futurelet\next\nextiii@}%
  \else\let\next\nextiv@\fi\next}%
 \def\nextiv@{\vnonvmode@
  {\ifmid@\let\next\midinsert\else\let\next\topinsert\fi
  \next\vbox to\thespace@{}\endinsert}
  {\ifmid@\nonvmodeerr@\midspace\else\nonvmodeerr@\topspace\fi}}%
 \def\nextiii@{\ifx\next\captionwidth\let\next\nextv@
  \else\let\next\nextvi@\fi\next}%
 \def\nextv@\captionwidth##1##2{\smallcaptionwidth@##1\relax\nextvi@{##2}}%
 \def\nextvi@##1{\def\thecaption@{##1}%
  \def\next@{\ifx\next\space@\def\next. {\futurelet\next\nextvii@}\else
   \def\next.{\futurelet\next\nextvii@}\fi\next.}%
  \futurelet\next\next@}%
 \def\nextvii@{\vnonvmode@
  {\ifmid@\let\next\midinsert\else
  \let\next\topinsert\fi\next\vbox to\thespace@{}\nobreak\smallskip
  \setbox\z@\hbox{\noindent\ignorespaces\thecaption@\unskip}%
  \ifdim\wd\z@>\smallcaptionwidth@\centerline{\vbox{\hsize\smallcaptionwidth@
  \noindent\ignorespaces\CorrectCounter\thecaption@
  \gdef\CorrectCounter{}\unskip}}%
  \else\centerline{\box\z@}\fi\endinsert}
  {\ifmid@\nonvmodeerr@\midspace
  \else\nonvmodeerr@\topspace\fi}}%
 \futurelet\next\next@}
% END OF \ins@ MODIFICATION
%
%
%      **************************
%      *     INITIALIZATION     *
%      **************************
\Input{\jobname.aux}
\immediate\openout\@auxout=\jobname.aux
\immediate\write\@auxout{\string\relax}
\catcode`\@=\active

